Horn Binary Serialization Analysis

A bit layout is a sequence of fields of certain bit lengths that specifies how to interpret a serial stream, e.g., the MP3 audio format. A layout with variable length fields needs to include meta-information to help the parser interpret unambiguously the rest of the stream; e.g. a field providing the length of a following variable length field. If no such information is available, then the layout is ambiguous. I present a linear-time algorithm to determine whether a layout is ambiguous or not by modelling the behaviour of a serial parser reading the stream as forward chaining reasoning on a collection of Horn clauses.

==> eptcsdata.tex <==
\providecommand{\firstpage}{56}
\providecommand{\publicationstatus}{J. P. Gallagher and P. R\"ummer (Eds.): 3rd Workshop\\
on Horn Clauses for Verification and Synthesis (HCVS)\\
EPTCS 219, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.219.6}{10.4204/EPTCS.219.6}}
\pdfoutput=1

